CADIS: Handling Cluster-skewed Non-IID Data in Federated Learning with Clustered Aggregation and Knowledge DIStilled Regularization

Federated learning enables edge devices to train a global model collaboratively without exposing their data. Despite achieving outstanding advantages in computing efficiency and privacy protection, federated learning faces a significant challenge when dealing with non-IID data, i.e., data generated by clients that are typically not independent and identically distributed. In this paper, we tackle a new type of Non-IID data, called cluster-skewed non-IID, discovered in actual data sets. The cluster-skewed non-IID is a phenomenon in which clients can be grouped into clusters with similar data distributions. By performing an in-depth analysis of the behavior of a classification model's penultimate layer, we introduce a metric that quantifies the similarity between two clients' data distributions without violating their privacy. We then propose an aggregation scheme that guarantees equality between clusters. In addition, we offer a novel local training regularization based on the knowledge-distillation technique that reduces the overfitting problem at clients and dramatically boosts the training scheme's performance. We theoretically prove the superiority of the proposed aggregation over the benchmark FedAvg. Extensive experimental results on both standard public datasets and our in-house real-world dataset demonstrate that the proposed approach improves accuracy by up to 16% compared to the FedAvg algorithm.

==> algo/clustering.tex <==
\begin{algorithm}[t]
    \caption{{\textbf{CADIS Training Algorithm}}}
    \label{algo:clustering}
    \small
    \Input{$n$: the total number of clients; $k$: the number of clients participating in each communication round.}
    Server initiates the global model $\omega_g^{0}$, and the similarity matrix\\
    \For{a communication round $\tau$ from $0$ to $T$}{
        Server selects $k$ clients randomly and sends $k$ copies of $w_g^{\tau}$ to them. \\
        % Selects $k$ clients randomly;\\
        % Sends $k$ copies of $w_g^{\tau}$ to the selected clients;\\
        \For{each client $C_i$ \textbf{in parallel}}{
            $\omega_{i}^{(\tau,0)} \gets \omega_g^{\tau}$  \\
            Local training in $E$ epochs with local data $D_i$:\\
            % $\mathcal{L} = \frac{1}{|D_i|}\sum_{e=1}^{E}\sum_{i = 1}^{\frac{n_k}{b}} (l_i(w_{k}^{(t,i)}) + \lambda r_i(w_{k}^{(t,i)}, w^t))$\\
            $\mathcal{L} \gets$ Computed using Formula (\ref{eqn:final_loss})\\
            $\omega_i^{\tau} \gets \omega_g^{\tau} - \eta_\tau.\nabla \mathcal{L}$ \\
            $C_i$ sends $\omega_i^{\tau}$ to the server;\\
        }
        Server computes client similarities based on the penultimate layer using Formula (\ref{eqn:sim}); \\
        updates the similarity matrix and rescaling to obtain the $Q$-matrix;  \\
        partition clients into clusters; \\
        computes the impact factors $\alpha^{\tau}_i$ for each client $C_i$; \\
        performs weighted aggregation: \\
        $\omega_g^{\tau+1} \gets \sum_{i=1}^{k}{\alpha^{\tau}_i \omega_i^{\tau}}$    
    }
\end{algorithm}

==> algo/compute-pdf.tex <==
\begin{algorithm}[t]
    \caption{{\textbf{Gaussian-kernel PDF transformation}}}
    \label{algo:pdf}
    \small
    \Input{Batch of representations $X$.}
    Compute the norm matrix $\mathcal{N} = \{\|r_i,r_j\|_2\}$, $\forall r_i, r_j \in X$; \\
    Compute the bandwidth $h \gets$ variance of $\mathcal{N}$;\\
    Compute the mean $\mu \gets$ mean of $\mathcal{N}$; \\
    Apply Gaussian kernel, compute matrix $G = e^{-\frac{(\mathcal{N} - \mu)^2}{h}}$;\\
    Normalize matrix $G = \frac{G}{\sum_{row}(G)}$;\\
    \Output{Gaussian matrix $G$}
\end{algorithm}

==> cluster-skew.tex <==
\label{sec:cluster-skew}

\textcolor{red}{Describe the intuition about the impacts of cluster-skew bias.
Present the experimental results comparing the use of FedAvg and cluster-based aggregation.}

\textcolor{blue}{This question is already discussed in \cite{zhang2021survey}. Should we mentioned it in Introduction rather than a separate section ?}

==> pen_proof1.tex <==
\subsubsection{The behavior of penultimate layer's gradient}
\label{appendix:pen_1}
Let $R = R(x) \in \mathbb{R}^u$ denote the representation of $x$ and $W \in \mathbb{R}^{u \times v}$ denote the parameter of the penultimate layer. Since most of activation functions return positive outputs (e.g sigmoid, ReLU), we assume that $R_i > 0$, $\forall i$. The logits vector of $x$ is denoted as $l(x) \in \mathbb{R}^v$ and can be computed as: 
\begin{equation}
    l(x) = W \cdot r = \begin{bmatrix}
       R_1 w_{11} + R_2 w_{12} + \dotsc + R_u w_{1u}           \\[0.3em]
       R_1 w_{21} + R_2 w_{22} + \dotsc + R_u w_{2u}           \\[0.3em]
       \vdots\\[0.3em]
       R_1 w_{v1} + R_2 w_{v2} + \dotsc + R_u w_{vu}
     \end{bmatrix}.
\end{equation}
From which, the probability of sample $x$ to be classified into label $j$ can be computed as:
\begin{equation}
    p_x(y = j) = \frac{e^{l_j}}{\sum_{i} e^{l_i}}.
\end{equation}
Suppose we adopt a vanilla training process where a cross entropy loss is applied for classification. Therefore, the classification loss is computed as:
\begin{equation}
    \mathcal{L}(p(x), y) = \sum_{i=0}^{v} {y_i log\bigg(\frac{1}{p_i(x)}\bigg)}.
\end{equation}
We then can deduce the gradient of an element $w_{zc} \in W$ with respect to the classifier loss $\mathcal{L} = \mathcal{L}(p(x), y)$:
\begin{equation}
    \frac{\partial \mathcal{L}}{\partial w_{zc}} = \frac{\partial L}{\partial l_k} \cdot 
    \frac{\partial l_k}{ \partial w_{zc}}.
    \label{eqn:grad}
\end{equation}
In which,
\begin{align}
    \frac{\partial \mathcal{L}}{\partial l_k} 
    &= 
    \begin{cases}
        -\frac{1}{ln(10)} \frac{y_j}{p_j(x)} p_j(x)(1-p_k(x))& \text{if $k = j$}\\
        \frac{1}{ln(10)} \frac{y_j}{p_j(x)} p_j(x) p_k(x)& \text{if $k \neq j$}\\
    \end{cases} \nonumber\\
    &= 
    \begin{cases}
        -\frac{1}{ln(10)} y_j (1-p_k(x)) & \text{if $k = j$} \\
        \frac{1}{ln(10)} y_j p_k(x) & \text{if $k \neq j$}\\
    \end{cases}
    \label{eqn:deriv_1}
\end{align}
is the partial derivative of the element $l_k$ in $l$ w.r.t $\mathcal{L}$ and the partial derivative of $w_{zc}$ from $l_k$ is simply:
\begin{equation}
    \frac{\partial l_k}{ \partial w_{zc}} = R_c.
    \label{eqn:deriv_2}
\end{equation}
From \ref{eqn:deriv_1} and \ref{eqn:deriv_2}, we can express \ref{eqn:grad} as:
\begin{equation}
    \frac{\partial \mathcal{L}}{\partial w_{zc}} = 
    \begin{cases}
        -\frac{1}{ln(10)} y_j (1-p_j(x)) R_c & \text{for row $j$} \\
        \frac{1}{ln(10)} y_j p_k(x) R_c & \text{for row $k \neq j$}\\
    \end{cases}.
    \label{eqn:full_grad}
\end{equation}

Because $y_j = 1$, $p_i(x) > 0$ and $r_c > 0,  \forall i, c$, by applying the gradient descent, it is obvious that the value of parameters on row $j$ of $W$ increase whereas that of the parameters on all other rows decreases.
The proof is complete.

==> pen_proof2.tex <==
\subsubsection{The consistency of penultimate layer and data distribution}
\label{appendix:pen_2}
Without the loss of generality, let label $p \notin G$, we consider the change of value of parameters on row $t$ of the penultimate layer, i.e $w_t$ and $w'_t$.

As proven in \textit{proposition \ref{prop:pen_shift}}, the partial derivative of $w_{ti}$ w.r.t the total loss when training a sample $(x, y), y\neq t$ is $\frac{1}{ln(10)} y_j p_t(x) r_i > 0$. After backpropagating through $d$ for a single epoch, the final value $w'_{ti}$ then can be computed as:
\begin{equation*}
    w'_{ti} \gets w_{ti} - \frac{\eta}{ln(10)} 
    \sum_{(x, j) \in d}
    y_j p_t(x) r_i.
\end{equation*}
Hence, the difference:
\begin{equation}
    \Delta w_{ti} = w'_{ti} - w_{ti} = - \frac{\eta}{ln(10)} 
    \sum_{(x, j) \in d}
    y_j p_t(x) r_i < 0.
\end{equation}
This property applies for all label $t \notin G$. The proof is complete.

==> penultimate_layer.tex <==
\label{sec:penultimate_layer}

% \subsection{Notations}
% In this section, we highlight some notations used throughout this paper. 

% \subsection{What Penultimate Layer Tells Us about The Data?}
\label{subsec:penultimate_characteristic}
% \textcolor{red}{Present the theoretical analysis concerning the gradient of the Penultimate Layer.}

Let us consider a standard classification task in which the neural network is composed of two successive components: the feature extractor (encoder) and the classifier (decoder), as depicted in Figure~\ref{fig:my_model}. For simplicity, the classifier consists of a dense layer only whereas the feature extractor can be designed using a variety of architectures.

We then sample an input $(x, y)$ where $x$ is the data and $y$ is the corresponding groundtruth label, in this specific case, $y = j$. For convenience, we encode $y$ as a one-hot vector whose $j$ element $y_j$ is marked $1$, elsewhere $0$.

\begin{proposition}
\label{prop:pen_shift}
Given the parameter matrix $W$ of the penultimate layer constructed from $v$ rows with $v$ is number of outputs (classes), and a sample $(x, y)$ whose groundtruth label is $j$, i.e. $y=j \in [1, v]$. Then after the training process the value of parameters on row $j$ of $W$ increases while that of other rows decreases.
\end{proposition}

\begin{proof}
See Appendix~\ref{appendix:pen_1}
\end{proof}

This insight from \textit{proposition \ref{prop:pen_shift}} helps uncovering some key aspects about the data set on which the model was trained on, especially the labels of the trained data set. Let $\mathcal{D} := \{(n_i, g_i)\}|i \in [1, m]$ denote the data set with $m$ labels where $n_i$ is the number of samples of class $g_i$. 

\begin{proposition}
Given data set $d \subset \mathcal{D}$, $d := \{(n_i, g_i)\}$, and its label set $G := \{g_i\}$ where $|d| < m$. And the penultimate layer of the model before being trained $(W)$ and after being trained $(W')$ on $d$. With $w_{kc} \in W$ and $w'_{kc} \in W'$ then $\Delta w_{kc} = w'_{kc} - w_{kc} < 0$ $\forall k \notin G$.
\label{prop:general}
\end{proposition}

\begin{proof}
See Appendix~\ref{appendix:pen_2}
\end{proof}

The intuition from \textit{proposition \ref{prop:general}} is that \textbf{\textit{when we observe the cumulative gradients of each row of the penultimate layer's parameter matrix, if on row $i$ exists any positive value then the data set on which the model was trained must contains samples of label $i$}}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/classification_model.eps}
    \caption{Standard neural network for classification task}
    \label{fig:my_model}
\end{figure}

\begin{figure*}[t]
 \centering
 	\subfigure[Single-class training]{
 	 \centering
    \includegraphics[width=0.3\textwidth]{fig/Single_label_analysis.eps}
    \label{fig:single_class}
    }
 	\subfigure[Double-class training]{
 	 \centering
    \includegraphics[width=0.3\textwidth]{fig/Double_label_analysis.eps}
    \label{fig:double_class} 
 	 }
 	\subfigure[Multi-class training]{
 	 \centering
    \includegraphics[width=0.3\textwidth]{fig/Multi_label_analysis.eps}
    \label{fig:multi_class} 
 	 }
 	 %\vspace{-0.2cm}
 	 \caption{The behavior of penultimate layer at different training scenarios. In single class scenarios, the cumulative gradients of the parameters on the row of the trained class, i.e. $0$ or $8$, is strictly non-negative whereas that of others is non-positive. In double-class scenarios, there exists both positive and negative cumulative gradients on the row of the trained classes, however, the gradients of the untrained classes remain strictly non-positive. The same observation applies for multi-class scenarios and the more the involving classes, the greater the negative values. 
 	 } 
 	 
 	 %\vspace{-0.2cm}
 \end{figure*}

==> tab/accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\usepackage[normalem]{ulem}
%\useunder{\uline}{\ul}{}

\begin{table*}[t]
	\caption{\small
	Comparison of top-1 test accuracy to baseline approaches with different partitioning methods, i.e., PA, BC, UC, MC.
	The values show the best accuracy that each FL method reaches during training. The best performance results are highlighted in the bold, underlined font.} %\emph{impr.(a)} and \emph{impr.(b)} are the relative accuracy improvement of FedDRL compared with the best and the worst baseline FL method (in percentage), respectively.  Significant improvements, i.e., $>1\%$, are also marked in the bold, underlined font.} 
	\label{table:accuracy}
	\centering
	\scriptsize
	\setlength\tabcolsep{4pt} % default value: 6pt
	\resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}cl|llll|llll|llll@{}}
    \toprule
    \multicolumn{2}{l}{}
    & \multicolumn{4}{c}{\textbf{MNIST}}
    & \multicolumn{4}{c}{\textbf{CIFAR-10}}
    & \multicolumn{4}{c}{\textbf{CIFAR-100}}\\
    \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
    \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Partitioning \\method\end{tabular}}
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC} & \multicolumn{1}{c}{MC}       
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC} & \multicolumn{1}{c}{MC} 
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC}
    & \multicolumn{1}{c}{UC} & \multicolumn{1}{c}{MC} \\ 
    \midrule
    \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}10\\  clients\end{tabular}}  
    & SingeSet 
    & 98.49 & 99.02 & 98.93 & 99.24
    & 66.28& 75.91& 79.52& 77.35& 52.24& 43.67& 48.13& 54.84
    \\
    \cmidrule(lr){3-14}
    & FedAvg   
    & 84.82 & 84.18 & 87.4 & 91.21
    & 47.73& 28.42& 33.86& 28.43& 34.67& 20.85& 25.69& 34.08
    \\
    & FedProx  
    & 85.06 & 83.37 & 86.71 & 90.67
    & 47.28& 28.53& 33.21& 28.55& 34.08& 20.94& 24.88& 33.47 
    \\
    & FedFA
    & 94.46 & 92.21 & 92.27 & 94.32
    & 52.39& 26.53& 34.63& 29.73& 39.58& 24.94& 27.16& 37.04
    \\
    & FedFV
    & 94.2 & 91.94 & 92.56 & 94.5
    & 52.44& 25.27& 33.40& 27.03& 39.64& 25.12& 27.25& 37.17
    \\
    & FedDyn
    & \textbf{\underline{95.59}} & \textbf{\underline{98.48}} & \textbf{\underline{98.00}} & \textbf{\underline{98.79}}
    & \textbf{\underline{55.27}}& 22.59& 44.77& 42.27& 40.78& 34.97& 35.54& 40.58
    \\
    & Cadis
    & 93.96 & 95.98 & 95.75 & 96.35
    & 52.70& \textbf{\underline{49.24}}& \textbf{\underline{50.62}}& \textbf{\underline{50.00}}& 39.33& 31.35& 33.71& 40.42
    \\
    %\cmidrule(lr){3-14}
    %& \emph{impr.(a)} 
    %& -1.71 & -2.54 & -2.30 & -2.47
    %& - & - & - & -
    %& - & - & - & - \\
    %& - \\
    %& \emph{impr.(b)} 
    %& 10.78 & 15.13 & 10.43 & 6.26
    %    & - & - & - & -
    %& - & - & - & - \\
    \midrule
    \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}100\\  clients\end{tabular}}  
    & SingeSet 
    & 99.22 & 99.24 & 99.18 & 99.15
    & 81.37& 39.20& 84.75& 82.11& 80.85& 52.66& 52.62& 52.36
    \\
    \cmidrule(lr){3-14}
    & FedAvg   
    & \textbf{\underline{96.89}} & 96.69 & 96.02 & 93.04
    & 62.26& 20.22& 43.45& 48.74& 21.01& 34.96& 34.16& 33.42
    \\
    & FedProx  
    & 96.73 & 96.66 & 96.01 & 92.91
    & 62.63& 20.18& 43.86& 48.43& 20.76& 34.61& 34.06& 33.21
    \\
    & FedFA
    & 96.5 & 96.67 & \textbf{\underline{96.29}} & 93.33
    & \textbf{\underline{66.41}}& 10.00& 10.00& 10.00& 1.00& 37.18& 37.38& 36.49
    \\
    & FedFV
    & 96.65 & 96.68 & 95.92 & 93.3
    & 66.21& 20.62& 31.16& 52.41& 24.31& 37.63& 37.33& 36.29
    \\
    & FedDyn
    & 92.79 & 93.36 & 91.72 & 88.04
    & 18.79& 19.34& 19.28& 19.62& 2.14& 9.69& 13.75& 5.39 
    \\
    & Cadis
    & 96.53 & \textbf{\underline{96.74}} & 96.02 & \textbf{\underline{93.45}}
    & 62.93& \textbf{\underline{34.83}}& \textbf{\underline{47.42}}& 50.09%
    & 17.75& 30.65& 31.35& 38.09
    \\
    %\cmidrule(lr){3-14}
    %& \emph{impr.(a)} 
    %& -0.37 & 0.05 & -0.28 & 0.13
    %& - & - & - & -
    %& - & - & - & - \\
    %%& - \\
    %& \emph{impr.(b)} 
    %& 4.03 & 3.62 & 4.69 & 6.14
    %    & - & - & - & -
    %& - & - & - & - \\
    \bottomrule
    \end{tabular}
    }
\end{table*}

==> tab/accuracy_other_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\usepackage[normalem]{ulem}
%\useunder{\uline}{\ul}{}

\begin{table}[t]
	\caption{\small
	Comparison of top-1 test accuracy to the benchmarks with different partitioning methods, i.e., PA, BC, UC.}
	\label{table:accuracy}
	\centering
	\scriptsize
	\setlength\tabcolsep{3pt} % default value: 6pt
	\resizebox{\linewidth}{!}{%
	%\begin{threeparttable}
    \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
    \toprule
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Partitioning \\method\end{tabular}}
    & \multicolumn{3}{c}{\textbf{MNIST}}
    & \multicolumn{3}{c}{\textbf{CIFAR-10}}
    & \multicolumn{3}{c}{\textbf{CIFAR-100}}\\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC} 
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC} 
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC}  \\ 
    \midrule
    SingeSet 
    & 99.18 & 99.22. & 99.17
    & 80.84 & 35.06 & 84.75 
    & 80.84 & 51.98 & 52.02 
    \\
    \cmidrule(lr){2-10}
    FedAvg   
    & 92.84 & \textbf{\textcolor{red}{95.68}} & \textbf{\textcolor{blue}{95.30}}
    & 60.55 & \textbf{\textcolor{blue}{19.90}} & \textbf{\textcolor{blue}{30.19}} 
    & 19.89 & 34.26 & 33.21 
    \\
    FedProx  
    & 92.88 & \textbf{\textcolor{blue}{95.66}} & 95.28
    & 60.73 & 19.88 & 30.03 
    & 19.71 & 33.93 & 33.43 
    \\
    FedFA
    & \textbf{\textcolor{blue}{95.64}} & 95.63 & \textbf{\textcolor{red}{95.40}}
    & \textbf{\textcolor{red}{65.36}} & 10 & 10 
    & 1.00 &  35.51 & 36.18
    \\
    FedDyn
    & 86.99 & 86.78 & 87.27
    & 11.64 & 11.81 & 12.08 
    & 1.17 & 2.18 & 2.73 
    \\
    CADIS
    & \textbf{\textcolor{red}{95.95}} & 95.46 & 95.07
    & \textbf{\textcolor{blue}{61.88}} & \textbf{\textcolor{red}{31.10}} & \textbf{\textcolor{red}{38.89}} 
    & 17.47 & 30.35 & 31.11 
    \\
    %\cmidrule(lr){3-14}
    %& \emph{impr.(a)} 
    %& -0.37 & 0.05 & -0.28 & 0.13
    %& - & - & - & -
    %& - & - & - & - \\
    %%& - \\
    %& \emph{impr.(b)} 
    %& 4.03 & 3.62 & 4.69 & 6.14
    %    & - & - & - & -
    %& - & - & - & - \\
    \bottomrule
    \end{tabular}
    %\begin{tablenotes}
     % \scriptsize
      %\item (*) The best results are highlighted in the \textbf{\textcolor{red}{bold-red}} font.
    %\end{tablenotes}
    %\end{threeparttable}
    }
\end{table}

==> tab/accuracy_other_raw.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\usepackage[normalem]{ulem}
%\useunder{\uline}{\ul}{}

\begin{table}[t]
	\caption{\small
	Comparison of top-1 test accuracy to the benchmarks with different partitioning methods, i.e., PA, BC, UC.}
	\label{table:accuracy}
	\centering
	\scriptsize
	\setlength\tabcolsep{3pt} % default value: 6pt
	\resizebox{\linewidth}{!}{%
	%\begin{threeparttable}
    \begin{tabular}{@{}l|ccc|ccc|ccc@{}}
    \toprule
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Partitioning \\method\end{tabular}}
    & \multicolumn{3}{c}{\textbf{MNIST}}
    & \multicolumn{3}{c}{\textbf{CIFAR-10}}
    & \multicolumn{3}{c}{\textbf{CIFAR-100}}\\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC} 
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC} 
    &  \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{BC} & \multicolumn{1}{c}{UC}  \\ 
    \midrule
    SingeSet 
    & 99.22 & 99.24 & 99.18 %& 99.15
    & 81.37& 39.20& 84.75 %& 82.11
    & 80.85& 52.66& 52.62 %& 52.36
    \\
    \cmidrule(lr){2-10}
    FedAvg   
    & \textbf{\textcolor{red}{96.89}} & 96.69 & 96.02 %& 93.04
    & 62.26& 20.22& 43.45 %& 48.74
    & \textbf{\textcolor{red}{21.01}}& 34.96& 34.16 %& 33.42
    \\
    FedProx  
    & 96.73 & 96.66 & 96.01 %& 92.91
    & 62.63& 20.18& 43.86 %& 48.43
    & 20.76& 34.61& 34.06 %& 33.21
    \\
    FedFA
    & 96.5 & 96.67 & \textbf{\textcolor{red}{96.29}} %& 93.33
    & \textbf{\textcolor{red}{66.41}}& 10.00& 10.00 %& 10.00
    & 1.00& \textbf{\textcolor{red}{37.18}}& \textbf{\textcolor{red}{37.38}} %& 36.49
    \\
    FedDyn
    & 92.79 & 93.36 & 91.72 %& 88.04
    & 18.79& 19.34& 19.28 %& 19.62
    & 2.14& 9.69& 13.75 %& 5.39 
    \\
    CADIS
    & 96.53 & \textbf{\textcolor{red}{96.74}} & 96.02 %& \textbf{\underline{93.45}}
    & 62.93& \textbf{\textcolor{red}{34.83}}& \textbf{\textcolor{red}{47.42}} %& 50.09%
    & 17.75& 30.65& 31.35 %& 38.09
    \\
    %\cmidrule(lr){3-14}
    %& \emph{impr.(a)} 
    %& -0.37 & 0.05 & -0.28 & 0.13
    %& - & - & - & -
    %& - & - & - & - \\
    %%& - \\
    %& \emph{impr.(b)} 
    %& 4.03 & 3.62 & 4.69 & 6.14
    %    & - & - & - & -
    %& - & - & - & - \\
    \bottomrule
    \end{tabular}
    %\begin{tablenotes}
     % \scriptsize
      %\item (*) The best results are highlighted in the \textbf{\textcolor{red}{bold-red}} font.
    %\end{tablenotes}
    %\end{threeparttable}
    }
\end{table}

==> tab/approaches.tex <==
% \begin{table*}[t]
% \centering
% \caption{Comparison between approaches}
% \label{tab:related}
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multirow{2}{*}{Approaches} & \multirow{2}{*}{Local training} & \multirow{2}{*}{Server aggregation} & \multicolumn{2}{c|}{Adaptivity}          \\ \cline{4-5} 
%   &       &           & \multicolumn{1}{l|}{Learning} & \multicolumn{1}{l|}{Semi-learning} \\ \hline
% FedAvg \cite{fedavg_mcmahan2017communication}       &   baseline  &    \cmark     &     &    \\ 
% FedProx \cite{fedprox_li2020federated}       & \cmark   &    baseline     &     &          \\ 
% FedFA   \cite{fedfa}       &    & \cmark       & \cmark &          \\ 
% FedFV  \cite{fedfv_wang2021federated}        &    & \cmark       & \cmark &          \\ 
% FedDyn  \cite{feddyn_acar2021federated}       & \cmark   & \cmark       & \cmark &          \\ 
% Proposal       & \cmark   & \cmark       &     & \cmark      \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\centering
\caption{Comparison between approaches}
\label{tab:related}
\begin{tabular}{|l|c|c|c|c|}
\hline
Algorithms & Local training & Server aggregation & Learning  \\
\hline
FedAvg \cite{fedavg_mcmahan2017communication}    &      baseline   &      \cmark     &           \\
FedProx \cite{fedprox_li2020federated}   &    \cmark    &     baseline     &           \\
FedFA \cite{fedfa_huang2020fairness}     &                &    \cmark    &     \cmark      \\
FedFV \cite{fedfv_wang2021federated} &               &   \cmark      &     \cmark    \\
FedDyn \cite{feddyn_acar2021federated}    &      \cmark   &       \cmark    &    \cmark \\
\textcolor{red}{CADIS (Our Proposal)}   &     \textcolor{red}{\cmark}    &     \textcolor{red}{\cmark}     &      \textcolor{red}{\cmark} \\
\hline
\end{tabular}
\end{table}

==> tab/notation.tex <==
\begin{table}[tb]
    \centering
    \caption{Notation}
    \label{tab:notate_tab}
    \begin{tabular}{|p{1.5cm}|p{6cm}|}
    \hline
    \textbf{Notation} & \textbf{Meaning}\\
    \hline
        $C_i$ & the $i$-th client\\
        $k$ & the number of clients in a communication round \\
        $\omega_i^{\tau}$ & the local trained model of client $i$ at round $\tau$ \\
        $\omega_g^{\tau}$ & the global model aggregated by server at round $\tau$ \\
        $W_i^\tau$ & the parameter matrix of the penultimate layer of client $C_i$'s local trained model at round $\tau$\\
        $W_g^\tau$ & the parameter matrix of the penultimate layer of the global model at round $\tau$\\
        $R(x)$ & representation of sample $x$\\
        $\mathcal{L}$ & loss function \\
        $s^{\tau}_{ij}$ & the instance similarity of $C_i$ and $C_j$ at round $\tau$\\
        %\emph{Similarity matrix} & A matrix whose each item $s_{ij}$ representing the cumulative similarity of client $C_i$ and $C_j$\\
        $Q$-matrix & the matrix obtained by applying min-max scaling on the similarity matrix \\
        $n_i$ & the number of samples owned by client $C_i$\\
        $N$ & total number of samples owned by all clients\\
        $m_\tau$ & the number of clusters in round $\tau$\\
        $M^{\tau}_{i}$ & the number of clients in the cluster containing client $C_i$ in round $\tau$\\
    \hline
    \end{tabular}
    \vspace{-15pt}
\end{table}

==> theo-Loss.tex <==
\subsubsection{Formulation of optimal loss function}
\label{appendix:loss_form}
Consider a federated learning situation where there are $3$ clients, denoted as $c_1, c_2$ and $c_3$ respectively. In which, client $c_1$ and $c_2$ are of the same cluster. For the sake of simplicity, we assume the followings are satisfied:
\begin{enumerate}
    \item The loss function used at client side is convex and have at least a minimum. For simplicity, we use the following simple one-dimensional function for any given $a_i$ and $b_i$:
    \begin{equation}
        f_i = a_i x^2 +b_ix, \text{  } a_i > 0, \text{  } \forall i.
    \end{equation}
    More specific, we choose arbitrarily the loss functions at the clients as:
    \begin{equation}
        \begin{cases}
            &f_1 = a_1 x^2 + b_1 x, \\
            &f_2 = a_2 x^2 + b_2 x, \\
            &f_3 = a_3 x^2 + b_3 x. \\
        \end{cases}
    \end{equation}
    
    % \begin{align*}
    %     &f_1 = a_1 x^2 + b_1 x, \\
    %     &f_2 = a_2 x^2 + b_2 x, \\
    %     &f_3 = a_3 x^2 + b_3 x. \\
    % \end{align*}
    However, since $c_1$ and $c_2$ are of the same cluster, their loss function are parameterized identically: $a_1 \approx a_2, b_1 \approx b_2 \to f_1 \approx f_2$.
    \item The number of samples at each client is the same.
\end{enumerate}

We now formulate the optimal loss function for Federated Learning in clustering scenarios. Consider a traditional training process in which we have a centralized data set $\mathcal{D}$ consists of samples from three classes, then we can express $\mathcal{D} := D_1 \cup D_2 \cup D_3$ where $D_i$ contains only data of class $i$. Thus, the total loss on $\mathcal{D}$ can be expressed as:
\begin{align}
    \mathcal{L}(\mathcal{D}) &= \frac{1}{|\mathcal{D}|}\sum_{(x,y)\in\mathcal{D}} L_\theta(x,y) \nonumber\\
    &= \frac{1}{|\mathcal{D}|} \sum_{D_i \in \mathcal{D}} \sum_{(x,y)\in D_i} L_\theta(x,y) \nonumber\\
    &\approx \frac{1}{|\mathcal{D}|} \Bigg(\sum_{D_i\in\mathcal{D}} |D_i| L(\bar{x}, i)\Bigg), \text{ $\bar{x} \in D_i$} \nonumber\\
    &\approx \sum_{D_i \in \mathcal{D}} \frac{|D_i|}{|\mathcal{D}|} L(\bar{x}, i)
    \label{eqn:fedavg_motiv}
\end{align}
Where $\bar{x}$ is an arbitrary sample from $D_i$. Equation~(\ref{eqn:fedavg_motiv}) gives the explanation of FedAVG approach. However, since we consider a clustering scenario, let $D_1 \equiv D_2$, meaning that both $D_1$ and $D_2$ contain samples of the same class, i.e. $1$. Then it is obvious that the loss function following Equation~(\ref{eqn:fedavg_motiv}) is biased towards class $1$ due to its overwhelming quantity of samples:
\begin{equation*}
    \mathcal{L}(\mathcal{D}) 
    \approx 
    \sum_{D_i \in \mathcal{D}} \frac{|D_i|}{|\mathcal{D}|} L(\bar{x}, i)
     \approx 
    \frac{2}{3} L(\bar{x}_1, 1) + \frac{1}{3} L(\bar{x}_3, 3).
\end{equation*}
Therefore, in our concern situation with loss functions $f_1, f_2$ and $f_3$, the unbiased loss function should be:
\begin{align}
    f &= L(\mathcal{D}) = \frac{1}{4} (f_1 + f_2) + \frac{1}{2} f_3 \nonumber\\
    &= \frac{1}{2} (a_1 + a_3) x^2 + (b_1 + b_3)x = \frac{1}{2} (a_1 + a_3) x^2.
    \label{eqn:optim_loss}
\end{align}
Here, we also omit the linear term $(b_1 + b_3)x$ by using a constraint $b_1 + b_3 = 0$ to simplify the computations. The calculation for the case $b_1 + b_3 \neq 0$ can be done with slightly more work. 

\subsubsection{Convergence of classifier loss}
\label{appendix:loss_convg}
In this section, on the basis of previous analysis, we give analysis on the convergence of the classifier loss, then we prove that FedSdiv results in lower classifier loss than FedAVG, in the case where $a_3 \geq a_1$, which often occurs as equality. Our analysis is constructed as follow:
\begin{enumerate}
    \item First, we compute the final model $y_{i}^{r,K}$ that client $c_i$ sends to the Server at the end of a communication round, given the initial model $x^r = y_i^{r,0}$.
    \item Next, we perform weighted aggregation according to algorithms (FedAVG and FedSdiv) to achieve the next initial model $x^{r+1}$.
    \item Recursively, we compute the final global model $x^R$ and its loss with respect to the optimal loss as in Equation~(\ref{eqn:optim_loss}).
    \item Then, We compare the loss of the model following FedAVG strategy and that following our proposal strategy, and prove that our proposal is superior.
\end{enumerate}

\textbf{Step 1:} Since the loss functions are congruent, without the loss of generality, we perform the analysis on a general case with index $i$:
\begin{itemize}
    \item Derivatives:
    \begin{equation}
        f'_i(z) = 2a_i z+ b_i.
    \end{equation}
    \item Recursive form of local updates, with learning rate $\eta_r$:
    \begin{align}
        y_i^{r,k} &= y_i^{r,k-1} - \eta_r \frac{d}{dz} \bigg(f(y_i^{r,k-1})\bigg), \forall i,r,k \nonumber\\
        &= y_i^{r,k-1} (1 - 2 a_i \eta_r) - \eta_r b_i \nonumber\\
        &= y_i^{r,k-2} (1 - 2 a_i \eta_r)^2 - \eta_r b_i (1 + (1 - 2a_i \eta_r)) \nonumber\\
        &= y_i^{r,k-3} (1 - 2 a_i \eta_r)^3 - \eta_r b_i (1 + (1 - 2a_i \eta_r)  \nonumber \\
        & + (1 - 2a_i \eta_r)^2) \nonumber
    \end{align}
    Thus, the recursive formula:
    \begin{equation}
        y_i^{r,k} = y_i^{r,k-t} (1 - 2 a_i \eta_r)^t - \eta_r b_i \sum_{\tau = 0}^{t-1} (1 - 2 a_i\eta_r)^\tau.
    \end{equation}
    We then compute the last model which client $i$ sends to the Server by substituting $k = K$ and note that $y_i^{r,0} = x^r$:
    \begin{equation}
        y_i^{r,K} = x^r (1 - 2 a_i \eta_r)^K - \eta_r b_i \sum_{\tau = 0}^{K-1} (1 - 2 a_i\eta_r)^\tau.
    \end{equation}
\end{itemize}

\textbf{Step 2:} We perform aggregation at Server according to the algorithm:
\begin{itemize}
    \item \textit{FedAvg}: the factors for losses are equal to $1/3$.
    \begin{align}
        x^{r+1} &= \sum_{i=1}^3 \alpha_i y_i^{r,k} \nonumber \\
        &= \frac{1}{3} \sum_{i=1}^3 \Bigg( x^r (1 - 2 a_i \eta_r)^K - \eta_r b_i \sum_{\tau = 0}^{K-1} (1 - 2 a_i\eta_r)^\tau \Bigg) \nonumber\\
        &= \frac{1}{3} x^r \sum_{i=1}^3 (1 - 2a_i\eta_r)^K - \frac{\eta_r}{3} \sum_{i=1}^3 b_i \sum_{\tau = 0}^{K-1} (1 - 2 a_i\eta_r)^\tau,
        \label{eqn:agg_avg_full}
    \end{align}
    where
    \begin{align}
        \frac{\eta_r}{3} \sum_{i=1}^3 b_i \sum_{\tau = 0}^{K-1} (1 - 2 a_i\eta_r)^\tau &=
        \frac{\eta_r}{3} \sum_{i=1}^3 b_i \frac{1 - (1 - 2a_i\eta_r)^K}{2a_i\eta_r} \nonumber\\
        &= \frac{1}{3} \sum_{i=1}^3 \frac{b_i}{a_i} \frac{1 - (1 - 2a_i\eta_r)^K}{2}.
    \end{align}
    Let $\phi_i = (1 - 2a_i\eta_r)^K$, we rewrite Equation~(\ref{eqn:agg_avg_full}) as:
    \begin{equation}
        x^{r+1} = \frac{1}{3} (2\phi_1 + \phi_3) x^r - \frac{1}{3}\Bigg(\frac{b_1}{a_1} (1-\phi_1) + \frac{b_3}{a_3} \frac{1-\phi_3}{2}\Bigg).
    \end{equation}
    
    \item \textit{FedSdiv}: the factors are $\{1/4,1/4,1/2\}$ respectively. Similarly, we have:
    \begin{align}
        x^{r+1} = \frac{1}{2}(\phi_1 + \phi_3)x^r - \frac{1}{2}\Bigg(\frac{b_1}{a_1}\frac{1 - \phi_1}{2} + \frac{b_3}{a_3}\frac{1-\phi_3}{2}\Bigg).
    \end{align}
\end{itemize}

\textbf{Step 3:} With the recursive form of $x^r$, we can compute the final aggregated model $x^R$ as:
\begin{align}
    x^R_{Avg} &= \Bigg(\frac{2\phi_1 + \phi_3}{3}\Bigg)^R x^0 \nonumber\\
    &- \Bigg(1-\bigg(\frac{2\phi_1 + \phi_3}{3}\bigg)^R\Bigg) 
    \frac{\frac{b_1}{a_1}(1-\phi_1) + \frac{b_3}{a_3} \frac{1-\phi_3}{2}}{3 - (2\phi_1 + \phi_3)} \\
    x^R_{Sdiv} &= \Bigg(\frac{\phi_1 + \phi_3}{2}\Bigg)^R x^0 \nonumber\\
    &- \Bigg(1-\bigg(\frac{\phi_1 + \phi_3}{2}\bigg)^R\Bigg)  \frac{\frac{b_1}{a_1}\frac{1-\phi_1}{2} + \frac{b_3}{a_3} \frac{1-\phi_3}{2}}{2 - (\phi_1 + \phi_3)}.
\end{align}

\textbf{Step 4:} Now, we use the optimal loss function~(\ref{eqn:optim_loss}) to evaluate the two approaches. At convergence ($R\to\infty$), the two models reduce to:
\begin{align}
    &x_{Avg} = \lim_{R\to\infty}x^{R}_{Avg} = \frac{\frac{b_1}{a_1}(1-\phi_1) + \frac{b_3}{a_3} \frac{1-\phi_3}{2}}{3 - (2\phi_1 + \phi_3)},\\
    &x_{Sdiv} = \lim_{R\to\infty}x^{R}_{Sdiv} = \frac{\frac{b_1}{a_1}\frac{1-\phi_1}{2} + \frac{b_3}{a_3} \frac{1-\phi_3}{2}}{2 - (\phi_1 + \phi_3)}.
\end{align}
Let $P = \frac{\phi_1 - 1}{\phi_1 + \phi_3 - 2}, Q = \frac{2\phi_1 -2}{2\phi_1 + \phi_3 - 3}$, the difference between the loss of FedAVG and that of our proposal is:
\begin{align}
    &\mathcal{L}_{Avg} - \mathcal{L}_{Sdiv}
    = \frac{1}{8} \frac{b_1^2}{a_1 a_3} (a_1+a_3)^2 v_1 v_2,
    % &=\frac{1}{8} (a_1 + a_3)((Q\beta_1 + (1-Q)\beta_2)^2- (P\beta_1 + (1-P)\beta_2)^2) \nonumber\\
    % &=\frac{1}{8} (a_1 + a_3) (Q-P)(\beta_1-\beta_3)(\beta_1(Q+P)+ \beta_3(2-Q-P))\nonumber\\
    \label{eqn:target}
\end{align}
where $v_1 = Q - P$ and $v_2 = \bigg(\frac{1}{a_1} + \frac{1}{a_3}\bigg)(Q+P) - \frac{2}{a_3}$. The rest of the proof focus on elaborating $\mathcal{L}_{Avg} > \mathcal{L}_{Sdiv}$.
Since $a_i > 0, \forall i, b_1^2 \neq 0$, we focus on the last two components $v_1, v_2$.
For $v_1$, we can prove this without trouble knowing that $\phi_i \in [0,1)$:
\begin{align}
    &v_1 = (\phi_1 - 1)\bigg(\frac{2}{2\phi_1 + \phi_3 - 3} - \frac{1}{\phi_1 + \phi_3 - 2}\bigg) \nonumber\\
    &= \frac{(\phi_1 - 1)(\phi_3 - 1)}{(2\phi_1 + \phi_3 - 3)(\phi_1 + \phi_3 - 2)} > 0.
\end{align}
To prove $v2 > 0$ needs a slightly more computing:
\begin{equation*}
    v_2 
    = \frac{1}{a_1}
    \Bigg(\bigg(1 + \frac{1}{\mu}\bigg)(Q+P) - \frac{2}{\mu}\bigg)\Bigg), \text{with $a_3 = \mu a_1$}.
\end{equation*}
Therefore we need to prove the following is true:
\begin{equation}
     \frac{(\phi_1 - 1)(4\phi_1 + 3\phi_3 -7)}{(2\phi_1 +\phi_3 - 3) (\phi_1 +\phi_3 -2)} - \frac{2}{\mu + 1} > 0
     \label{eqn:prof_1}
\end{equation}
Now, we denote $x_i = 1 - \phi_i > 0$, then:
\begin{align}
    &\frac{(\phi_1 - 1)(4\phi_1 + 3\phi_3 -7)}{(2\phi_1 +\phi_3 - 3) (\phi_1 +\phi_3 -2)} = \frac{x_1 (4x_1 + 3x_3)}{(x_1 +x_3)(2x_1 + x_3)} \nonumber\\
    &> \frac{2x_1}{x_1 + x_3} = \frac{2}{1 + \frac{x_3}{x_1}}.
    \label{eqn:prof_2}
\end{align}
Moreover, we also have:
\begin{align}
    &\frac{x_3}{x_1} = \frac{1 - (1 - 2 a_3\eta_r)^K}{1 - (1- 2 a_1 \eta_r)^K}
    = \frac{2a_3\eta_r\sum_{j=0}^{K-1} (1 -2a_3\eta_r)^j}{2a_1\eta_r \sum_{j=0}^{K-1} (1 -2a_1\eta_r)^j} \nonumber\\
    &= \mu \frac{\sum_{j=0}^{K-1} (1 -2a_3\eta_r)^j}{\sum_{j=0}^{K-1} (1 -2a_1\eta_r)^j}
    \leq \mu. 
    \label{eqn:prof_3}
\end{align}

From Equations~(\ref{eqn:prof_3}) and (\ref{eqn:prof_2}), the inequality~(\ref{eqn:prof_1}) holds. Which, together with Equation~(\ref{eqn:target}), complete our proof:
\begin{equation}
    \mathcal{L}_{Avg} > \mathcal{L}_{Sdiv}.
\end{equation}



==> theo-Qmatrix.tex <==
\subsubsection{Convergence rate of $Q$-matrix}
\label{appendix:Q_convg}
Let $N$ denote the total number of clients and $K$ is the number of clients participating in a communication round, then $K \leq N$. We give analysis on the convergence rate of $Q$-matrix when its entries are asynchronously updated. The matrix is assured full when all the clients are selected at least once. The problem is then reduced to: "\textit{Compute the necessary number of selection in average (each time $K$ elements) so that all $N$ elements are selected at least once}".

We denote $S_i$ $(\forall i \in [0, N])$ as a random variable representing the number of selection required for all the the elements to be selected at least once, if $i$ clients are already selected. Then we can compute the expected value of $S_0$ recursively as:
\begin{equation}
    \begin{cases}
        &E[S_0] = 1 + E[S_K], \\
        &E[S_1] = a_{10} (1 + E[S_K]) + a_{11} (1 + E[S_{K+1}]), \\
        &E[S_2] = a_{20} (1 + E[S_K]) + a_{21} (1 + E[S_{K+1}]) +\\
        &a_{22} (1 + E[S_{K+2}]), \\
        &\dots\\
        &E[S_i] = \sum_{j=0}^i a_{ij} (1 + E[S_{K+j}]),\\
        &\dots\\
        &E[S_N] = 0.
    \end{cases}
    \label{eqn:S0}
\end{equation}
In which, $a_{ij}$ is the transitioning probability from state $S_i$ to $S_{k+j}$, and is computed as:
\begin{equation}
    a_{ij} = \frac{C_{N-i}^{K+j-i} C_{i}^{i-j}}{C^K_N}.
    \label{eqn:a}
\end{equation}
Then we can substitute Equation~(\ref{eqn:a}) into Equation~(\ref{eqn:S0}) to compute the expected number of iteration required. We conduct extensive experiments to demonstrate the results of (\ref{eqn:S0}) in different settings, i.e. the total number of clients ranges from $10$ to $350$ while the participation rates are fixed at $0.2, 0.4, 0.6, 0.8$ and $1$. It is clearly shown in Figure~\ref{fig:convergence} that the expected iteration required for convergence of $Q$-matrix is trivial with respect to the number of communication round (i.e. $500$). For instance, when there are $100$ clients in total, $Q$-matrix is expected to be filled after roughly $25$ iterations at the participation rate of $20\%$ and after about $50$ iterations at the rate of $10\%$.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth, trim=0 3cm 0 3cm, clip]{fig/Q_convergence.eps}
    \caption{Estimations of required iterations for convergence of $Q$-matrix.}
    \label{fig:convergence}
\end{figure}
